Hybrid kT-factorization and impact factors at NLO

In the hybrid kT-factorization formula, one initial-state parton momentum is space-like and carries non-vanishing transverse components, while the other is on-shell. We promote this factorization formula to next-to-leading order. Studying the partonic cross section, we identify all soft and collinear divergencies in the real and virtual contribution, and recognize that all non-cancelling ones can be attributed to PDF evolution, evolution kernel, and target impact factors. In result, we construct a framework that may be used to compute NLO impact factors in general. In particular, we recover known expressions for inclusive NLO quark-and gluon impact factor corrections.

==> 17-intsub.tex <==
\section{Integral of the collinear subtraction}
\newcommand{\zM}{\bar{z}}
\newcommand{\yM}{\bar{y}}
\newcommand{\zP}{z}
\newcommand{\yP}{y}
\newcommand{\Qinst}{\myScript{Q}_{\inlbl}}
\newcommand{\Qbar}{\myScript{Q}_{\inbar}}
Consider the following type of collinear limit, re-distributing the whole recoil over the initial-state variables without approximation
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{multline}
\justMStar\big(\xPin,\kperp,\xMin\,;r,\{p_i\}_{i=1}^n\big)
\\
\overset{r\to\xP_r\pPA}{\longrightarrow}
\frac{1}{\lop{\xP_r\pPA}{r}}\,\frac{\Qinst(1-\xP_r/\xPin)}{1-\xP_r/\xPin}
\,\justMStar\big(\xPin-\xP_r,\kperp-\rperp,\xMin-\xM_r\,;\{p_i\}_{i=1}^n\big)
~.
\end{multline}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
Usually on would have $\Qinst(z)=(1-z)\Pinst(z)$ where $\Pinst$ is the splitting function, but with $\Qinst$ the following formulas will be a bit more compact.
%
Notice that the bar- and non-bar variables are treated equivalently in the \matrixelement\ on the right hand side.
%
Including phase space and integrating over the momentum $r$, we find (remember the flux factor)
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
&\dRfamColl\big(\xPin,\kperp,\xMin\,;\{p_i\}_{i=1}^n\big)
\notag\\&\hspace{2ex}=
    \frac{\cNLO}{\piep\mu^\vep}
    \frac{1}{|\kperp|^2}
    \int d^{4+\vep}r\,\delta(r^2)
    \,\theta(\xP_r<\xPin)\theta(\xM_r<\xMin)
    \,\frac{1}{\lop{\xP_r\pPA}{r}}
    \,\frac{\Qinst(1-\xP_r/\xPin)}{1-\xP_r/\xPin}
\\&\hspace{16ex}\times
    \,\frac{\xPin-\xP_r}{\xPin}
    \,\frac{\xMin-\xM_r}{\xMin}
    \,d\PSTstr_{n}\big(\xPin-\xP_r,\kperp-\rperp,\xMin-\xM_r\,;\{p_i\}_{i=1}^{n}\big)
    \,\JetB\big(\{p_i\}_{i=1}^{n}\big)
\notag
\end{align}
%
Using that $|\rperp|^2-2\xP_r\lop{\pPA}{r}=0$ we get
%
\begin{align}
&\dRfamColl\big(\xPin,\kperp,\xMin\,;\{p_i\}_{i=1}^n\big)
\notag\\&\hspace{2ex}=
    \frac{\cNLO}{\piep\mu^\vep}
    \frac{1}{|\kperp|^2}
    \int d^{4+\vep}r\,\delta(r^2)\,\frac{2}{|\rperp|^2}
    \,\theta(\xP_r<\xPin)\theta(\xM_r<\xMin)
    \,\frac{\Qinst(1-\xP_r/\xPin)}{1-\xP_r/\xPin}
\notag\\&\hspace{16ex}\times
    \frac{\xPin-\xP_r}{\xPin}
    \,\frac{\xMin-\xM_r}{\xMin}
    \,d\PSTstr_{n}\big(\xPin-\xP_r,\kperp-\rperp,\xMin-\xM_r\,;\{p_i\}_{i=1}^{n}\big)
    \,\JetB\big(\{p_i\}_{i=1}^{n}\big)
\notag\\&\hspace{2ex}=
    \frac{\cNLO}{\piep\mu^\vep}
    \int d^{4+\vep}r\,\delta(r^2)\,\frac{2}{|\rperp|^2}
    \,\frac{|\kperp-\rperp|^2}{|\kperp|^2}
    \,\theta(\xP_r<\xPin)\theta(\xM_r<\xMin)
    \,\Qinst(1-\xP_r/\xPin)
\notag\\&\hspace{16ex}\times
    \frac{\xMin-\xM_r}{\xMin}
    \,\frac{d\PSTstr_{n}\big(\xPin-\xP_r,\kperp-\rperp,\xMin-\xM_r\,;\{p_i\}_{i=1}^{n}\big)}
           {|\kperp-\rperp|^2}
    \,\JetB\big(\{p_i\}_{i=1}^{n}\big)
\notag\\&\hspace{2ex}=
    \frac{\cNLO}{\piep\mu^\vep}
    \int_0^{\xPin}d\xP_r\int_0^{\xMin} d\xM_r\int\frac{d^{2+\vep}\rperp}{|\rperp|^2}
    \,\frac{|\kperp-\rperp|^2}{|\kperp|^2}
    \,\delta\bigg(\xP_r\xM_r-\frac{|\rperp|^2}{\sTot}\bigg)
\\&\hspace{18ex}\times
    \,\Qinst(1-\xP_r/\xPin)
    \,(1-\xM_r/\xMin)
    \,\dBstar\big(\xPin-\xP_r,\kperp-\rperp,\xMin-\xM_r\,;\{p_i\}_{i=1}^{n}\big)
\notag\end{align}
%
Realize that
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\delta^4\bigg(\kin+\kinBar-r-\sum_{i=1}^np_i\bigg)
=
\delta^4\bigg((\xPin-\xP_r)\pPA+\kperp-\rperp+(\xMin-\xM_r)\pM-\sum_{i=1}^np_i\bigg)
~,
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
so the phase space in $\dBstar$ together with the integral over $r$ still comprises full $(n+1)$-momenta ``real-radiation'' phase space.
%
Also, it is clear that we can generalize the formula to include the other collinear limit case by inserting the symbol $\Qbar$, and deciding at a later stage in the calculation that one of $\Qinst,\Qbar$ is the actual relevant splitting function and the other one the identity function.
%
Thus we consider
%
\begin{align}
&\dRfamColl\big(\xPin,\kperp,\xMin\,;\{p_i\}_{i=1}^n\big)
\notag\\&\hspace{8ex}=
    \frac{\cNLO}{\piep\mu^\vep}
    \int_0^{\xPin}d\xP_r\int_0^{\xMin} d\xM_r\int\frac{d^{2+\vep}\rperp}{|\rperp|^2}
    \,\frac{|\kperp-\rperp|^2}{|\kperp|^2}
    \,\delta\bigg(\xP_r\xM_r-\frac{|\rperp|^2}{\sTot}\bigg)
\\&\hspace{16ex}\times
    \,\Qinst(1-\xP_r/\xPin)
    \,\Qbar(1-\xM_r/\xMin)
    \,\dBstar\big(\xPin-\xP_r,\kperp-\rperp,\xMin-\xM_r\,;\{p_i\}_{i=1}^{n}\big)
~.
\notag\end{align}
%
Now we put this underneath an integral over initial-state variables with an extra ``luminosity'' function $Ff(\xPin,\kperp,\xMin)$
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
I &= 
\int_0^1\frac{d\xPin}{\xPin}\int d^2\kperp\int_0^1\frac{d\xMin}{\xMin}
\,Ff(\xPin,\kperp,\xMin)
\,\dRfamColl\big(\xPin,\kperp,\xMin\,;\{p_i\}_{i=1}^n\big)
\notag\\&\hspace{0ex}=
    \frac{\cNLO}{\piep\mu^\vep}
    \int_0^{1}\frac{d\xPin}{\xPin}
    \int d^2\kperp
    \int_0^{1}\frac{d\xMin}{\xMin}
    \int_0^{\xPin}d\xP_r
    \int_0^{\xMin}d\xM_r
    \int\frac{d^{2+\vep}\rperp}{|\rperp|^2}
    \,\frac{|\kperp-\rperp|^2}{|\kperp|^2}
    \,\delta\bigg(\xP_r\xM_r-\frac{|\rperp|^2}{\sTot}\bigg)
\\&\hspace{2ex}\times
    \,Ff(\xPin,\kperp,\xMin)
    \,\Qinst(1-\xP_r/\xPin)
    \,\Qbar(1-\xM_r/\xMin)
    \,\dBstar\big(\xPin-\xP_r,\kperp-\rperp,\xMin-\xM_r\,;\{p_i\}_{i=1}^{n}\big)
\notag\end{align}
%
We will omit the arguments $\{p_i\}_{i=1}^{n}$ from now on.
%
Write $\xP_r=z\xPin$ and $\kperp\leftarrow\kperp+\rperp$ and $\xM_r=\zM\xMin$
%
\begin{align}
I&=
    \frac{\cNLO}{\piep\mu^\vep}
    \int_0^{1}\frac{d\xPin}{\xPin}
    \int d^2\kperp
    \int_0^{1}\frac{d\xMin}{\xMin}
    \int_0^{1}d\zP
    \int_0^{1}d\zM
    \int\frac{d^{2+\vep}\rperp}{|\rperp|^2}
    \,\frac{|\kperp|^2}{|\kperp+\rperp|^2}
    \,\delta\bigg(\zP\zM-\frac{|\rperp|^2}{\sTot\xPin\xMin}\bigg)
\\&\hspace{12ex}\times
    \,Ff(\xPin,\kperp+\rperp,\xMin)
    \,\Qinst(1-\zP)
    \,\Qbar(1-\zM)
    \,\dBstar\big((1-\xP)\xPin,\kperp,(1-\zM)\xMin\big)
\notag\end{align}
%
Now we introduce $\yP=(1-\zP)\xPin$ to replace the $\xPin$ integration, and $\yM=(1-\zM)\xMin$ to replace the $\xMin$
%
\begin{align}
I&=
    \frac{\cNLO}{\piep\mu^\vep}
    \int_0^{1}d\zP
    \int_0^{1}d\zM
    \int_0^{1-\zP}\frac{d\yP}{\yP}
    \int_0^{1-\zM}\frac{d\yM}{\yM}
    \int d^2\kperp
    \int\frac{d^{2+\vep}\rperp}{|\rperp|^2}
    \,\frac{|\kperp|^2}{|\kperp+\rperp|^2}
    \,\delta\bigg(\zP\zM-\frac{|\rperp|^2(1-\zP)(1-\zM)}{\sTot\yP\yM}\bigg)
\notag\\&\hspace{12ex}\times
    \,Ff\bigg(\frac{\yP}{1-\zP},\kperp+\rperp,\frac{\yM}{1-\zM}\bigg)
    \,\Qinst(1-\zP)
    \,\Qbar(1-\zM)
    \,\dBstar\big(\yP,\kperp,\yM\big)
\end{align}
%
Now we use the fact that the combined integration region for $z$ and $y$ is symmetric with respect to the diagonal, that is for general integrand $h$
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\int_0^1dz\int_0^{1-z}dy \,h(y,z) = \int_0^1dy\int_0^{1-y}dz\,h(y,z)
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
and the same for $\zM,\yM$, so
%
%
\begin{align}
I&=
    \frac{\cNLO}{\piep\mu^\vep}
    \int_0^{1}\frac{d\yP}{\yP}
    \int_0^{1}\frac{d\yM}{\yM}
    \int_0^{1-\yP}\!\!d\zP
    \int_0^{1-\yM}\!\!d\zM
    \int d^2\kperp
    \int\frac{d^{2+\vep}\rperp}{|\rperp|^2}
    \,\frac{|\kperp|^2}{|\kperp+\rperp|^2}
    \,\delta\bigg(\zP\zM-\frac{|\rperp|^2(1-\zP)(1-\zM)}{\sTot\yP\yM}\bigg)
\notag\\&\hspace{12ex}\times
    \,Ff\bigg(\frac{\yP}{1-\zP},\kperp+\rperp,\frac{\yM}{1-\zM}\bigg)
    \,\Qinst(1-\zP)
    \,\Qbar(1-\zM)
    \,\dBstar\big(\yP,\kperp,\yM\big)
\end{align}
%
Thus we find
%
\begin{equation}
I = 
\int_0^1\frac{d\xPin}{\xPin}\int d^2\kperp\int_0^1\frac{d\xMin}{\xMin}
\,\widetilde{Ff}(\xPin,\kperp,\xMin)\,\dBstar\big(\xPin,\kperp,\xMin\big)
\end{equation}
%
with
%
\begin{align}
\widetilde{Ff}(\xPin,\kperp,\xMin)&=
    \frac{\cNLO}{\piep\mu^\vep}
    \int_0^{1-\xPin}\!\!d\zP
    \int_0^{1-\xMin}\!\!d\zM
    \int\frac{d^{2+\vep}\rperp}{|\rperp|^2}
    \,\frac{|\kperp|^2}{|\kperp+\rperp|^2}
    \,\delta\bigg(\zP\zM-\frac{|\rperp|^2(1-\zP)(1-\zM)}{\sTot\xPin\xMin}\bigg)
\notag\\&\hspace{16ex}\times
    \,Ff\bigg(\frac{\xPin}{1-\zP},\kperp+\rperp,\frac{\xMin}{1-\zM}\bigg)
    \,\Qinst(1-\zP)
    \,\Qbar(1-\zM)
\end{align}
%
The $\delta$-function implies integration limits for $|\rperp|$.
%
For example, we have
%
\begin{align}
\delta\bigg(\zP\zM-\frac{|\rperp|^2(1-\zP)(1-\zM)}{\sTot\xPin\xMin}\bigg)
&=
\frac{1}{\zP}\,\delta\bigg(\zM-\frac{|\rperp|^2(1-\zP)(1-\zM)}{\sTot\xPin\xMin\zP}\bigg)
\notag\\&=
\frac{1}{\zP}\,\delta\bigg(\zM\bigg(1+\frac{|\rperp|^2(1-\zP)}{\sTot\xPin\xMin\zP}\bigg)-\frac{|\rperp|^2(1-\zP)}{\sTot\xPin\xMin\zP}\bigg)
\\&=
\frac{1}{\zP}\,\frac{\sTot\xPin\xMin\zP}{\sTot\xPin\xMin\zP+|\rperp|^2(1-\zP)}\,\delta\bigg(\zM-\frac{|\rperp|^2(1-\zP)}{\sTot\xPin\xMin\zP+|\rperp|^2(1-\zP)}\bigg)
\notag
\end{align}
%
implying the limit
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
&\frac{|\rperp|^2(1-\zP)}{\sTot\xPin\xMin\zP+|\rperp|^2(1-\zP)} < 1-\xMin
\quad\Leftrightarrow\quad
%\frac{|\rperp|^2}{\sTot\xPin\xMin\frac{\zP}{1-\zP}+|\rperp|^2} < 1-\xMin
%\notag\\&\Leftrightarrow\quad
%|\rperp|^2< \bigg(\sTot\xPin\xMin\frac{\zP}{1-\zP}+|\rperp|^2\bigg)(1-\xMin)
%\quad\Leftrightarrow\quad
|\rperp|^2< \sTot\xPin(1-\xMin)\frac{\zP}{1-\zP}
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
Notice that we could also have singled out the $z$ variable, and have the same formulas with the bar- and non-bar variables exchanged.
%
Let us however stick to the example above, and set
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\Qinst(1-\zP) = \frac{2\Nc}{1-\zP}
\;\;,\;\;
\Qbar(1-\zM) = 1-\zM
\;\;,\;\;
Ff(\xPin,\kperp,\xMin) = |\kperp|^2F(\xPin,\kperp)\,f(\xMin)
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
so we can write
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{multline}
\frac{\widetilde{Ff}(\xPin,\kperp,\xMin)}{|\kperp|^2}
=
    \frac{2\cNLO\Nc}{\piep\mu^\vep}
    \int_0^{1-\xPin}\frac{dz}{z(1-z)}
    \int\frac{d^{2+\vep}\rperp}{|\rperp|^2}
    \,\theta\bigg(|\rperp|^2 < \sTot\xPin(1-\xMin)\frac{\zP}{1-\zP}\bigg)
\\\times
    F\bigg(\frac{\xPin}{1-\zP},\kperp+\rperp\bigg)
    \bigg(\frac{\sTot\xPin\xMin\zP}{\sTot\xPin\xMin\zP+|\rperp|^2(1-\zP)}\bigg)^2
    f\bigg(\xMin+\frac{|\rperp|^2(1-\zP)}{\sTot\xPin\zP}\bigg)
~,
\end{multline}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
It is common formulate such integrals in terms of $z\leftarrow(1-z)$, but we prefer to keep the singularity at $z=0$ like this.
%
Let us remove the $z$-dependence of the integration limit by substituting $|\rperp|\leftarrow\sqrt{\srac{z}{1-z}}|\rperp|$.
%
We get
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{multline}
\frac{\widetilde{Ff}(\xPin,\kperp,\xMin)}{|\kperp|^2}
=
    \frac{2\cNLO\Nc}{\piep\mu^\vep}
    \int_0^{1-\xPin}\frac{dz}{z^{1-\vep/2}(1-z)^{1+\vep/2}}
    \int\frac{d^{2+\vep}\rperp}{|\rperp|^2}
    \,\theta\big(|\rperp|^2 < \sTot\xPin(1-\xMin)\big)
\\\times
    F\bigg(\frac{\xPin}{1-\zP},\kperp+\sqrt{\frac{z}{1-z}}\,\rperp\bigg)
    \bigg(\frac{\sTot\xPin\xMin}{\sTot\xPin\xMin+|\rperp|^2}\bigg)^2
    f\bigg(\xMin+\frac{|\rperp|^2}{\sTot\xPin}\bigg)
~,
\end{multline}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%




\newpage


or substituting $z\leftarrow1-z$
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{multline}
\widetilde{Ff}(\xPin,\kperp,\xMin)
=
    \frac{2\cNLO\Nc}{\piep\mu^\vep}
    \int_{\xPin}^1\frac{dz}{z(1-z)}
    \int\frac{d^{2+\vep}\rperp}{|\rperp|^2}\,\frac{|\kperp|^2}{|\kperp+\rperp|^2}
    \,\theta\bigg(|\rperp|^2 < \sTot\xPin(1-\xMin)\frac{1-z}{z}\bigg)
\\\times
    F\bigg(\frac{\xPin}{z},\kperp+\rperp\bigg)
%    \int_{\xMin}^1d\zM
%    \,\delta\bigg(\zM-\frac{\sTot\xPin\xMin(1-z)}{\sTot\xPin\xMin(1-z)+|\rperp|^2z}\bigg)
%    \,\zM^2\,f\bigg(\frac{\xMin}{\zM}\bigg)
    \bigg(\frac{\sTot\xPin\xMin(1-z)}{\sTot\xPin\xMin(1-z)+|\rperp|^2z}\bigg)^2
    f\bigg(\xMin+\frac{|\rperp|^2z}{\sTot\xPin(1-z)}\bigg)
~.
\end{multline}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
This integral seems divergent for both $|\rperp|\to$ and $z\to1$ independently, but the two are tied via the upper integration limit on $|\rperp|$.
%
Substituting $r\leftarrow\sqrt{1-z}\,r$, we find
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{multline}
\widetilde{Ff}(\xPin,\kperp,\xMin)
\\
=
    \frac{2\cNLO\Nc}{\piep\mu^\vep}
    \int_{\xPin}^1\frac{dz}{z(1-z)^{1-\vep/2}}
    \int\frac{d^{2+\vep}\rperp}{|\rperp|^2}\,\frac{|\kperp|^2}{|\kperp+\sqrt{1-z}\,\rperp|^2}
    \,\theta\bigg(|\rperp|^2 < \frac{\sTot\xPin(1-\xMin)}{z}\bigg)
\\\times
    F\bigg(\frac{\xPin}{z},\kperp+\sqrt{1-z}\,\rperp\bigg)
    \bigg(\frac{\sTot\xPin\xMin}{\sTot\xPin\xMin+|\rperp|^2z}\bigg)^2
    f\bigg(\xMin+\frac{|\rperp|^2z}{\sTot\xPin}\bigg)
~,
\end{multline}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
and we see that the singularities only happen at $|\rperp|\to0$.
%
Let us however return to the previous integral, and tame it in stages.
%
We write
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
&\widetilde{Ff}(\xPin,\kperp,\xMin)
\notag\\&\hspace{2ex}=
    \frac{2\cNLO\Nc}{\piep\mu^\vep}
    \int_{\xPin}^1\frac{dz}{z(1-z)}
    \int\frac{d^{2+\vep}\rperp}{|\rperp|^2}\,\frac{|\kperp|^2}{|\kperp+\rperp|^2}
    \,\theta\bigg(|\rperp|^2 < \sTot\xPin(1-\xMin)\frac{1-z}{z}\bigg)
\notag\\&\hspace{10ex}\times
    F\bigg(\frac{\xPin}{z},\kperp+\rperp\bigg)
    \bigg[
    \bigg(\frac{\sTot\xPin\xMin(1-z)}{\sTot\xPin\xMin(1-z)+|\rperp|^2z}\bigg)^2
    f\bigg(\xMin+\frac{|\rperp|^2z}{\sTot\xPin(1-z)}\bigg)
    - f(\xMin)\bigg]
\notag\\&\hspace{2ex}+
    \tilde{F}(\xPin,\kperp)\,f(\xMin)
\label{Eq:072}
~,
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
where 
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{multline}
\tilde{F}(\xPin,\kperp)=
    \frac{2\cNLO\Nc}{\piep\mu^\vep}
    \int_{\xPin}^1\frac{dz}{z(1-z)}
    \int\frac{d^{2+\vep}\rperp}{|\rperp|^2}\,\frac{|\kperp|^2}{|\kperp+\rperp|^2}
    \,\theta\bigg(|\rperp|^2 < \sTot\xPin(1-\xMin)\frac{1-z}{z}\bigg)
\\\times
    F\bigg(\frac{\xPin}{z},\kperp+\rperp\bigg)
\label{Eq:073}
~.    
\end{multline}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
The subtracted explicit integral in \Equation{Eq:072} is now finite for $\vep\to0$, and the singularities are contained in \Equation{Eq:073}.
%
Notice that \Equation{Eq:073} has the form of an evolution equation like Equation~(2.21) in~\cite{Nefedov:2020ecb}.
%
Now we write
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
\tilde{F}(\xPin,\kperp) &=
    \frac{2\cNLO\Nc}{\piep\mu^\vep}
    \int_{\xPin}^1\frac{dz}{z(1-z)}
    \int\frac{d^{2+\vep}\rperp}{|\rperp|^2}\,\frac{|\kperp|^2}{|\kperp+\rperp|^2}
    \,\theta\bigg(|\rperp|^2 < \sTot\xPin(1-\xMin)\frac{1-z}{z}\bigg)
\notag\\&\hspace{28ex}\times
    \bigg[F\bigg(\frac{\xPin}{z},\kperp+\rperp\bigg)
        -\frac{|\kperp+\rperp|^2}{|\kperp|^2}\,F\bigg(\frac{\xPin}{z},\kperp\bigg)
    \bigg]
\notag\\&\hspace{0ex}+\tilde{\tilde{F}}(\xPin,\kperp)
\label{Eq:074}
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
with
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
\tilde{\tilde{F}}(\xPin,\kperp)&=
    \frac{2\cNLO\Nc}{\piep\mu^\vep}
    \int_{\xPin}^1\frac{dz}{z(1-z)}
    \int\frac{d^{2+\vep}\rperp}{|\rperp|^2}
    \,\theta\bigg(|\rperp|^2 < \sTot\xPin(1-\xMin)\frac{1-z}{z}\bigg)
       \,F\bigg(\frac{\xPin}{z},\kperp\bigg)
\notag\\&\hspace{0ex}=
    \frac{4\cNLO\Nc}{\vep}\bigg(\frac{\sTot\xPin(1-\xMin)}{\mu^2}\bigg)^{\vep/2}
    \int_{\xPin}^1\frac{dz}{z(1-z)}
    \bigg(\frac{1-z}{z}\bigg)^{\vep/2}
   \,F\bigg(\frac{\xPin}{z},\kperp\bigg)
~.
\label{Eq:075}
\end{align}
%
Again, the subtracted explicit integral in \Equation{Eq:074} is finite for $\vep\to0$, and the singularities are contained in \Equation{Eq:075}.
%
We continue by writing
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\tilde{\tilde{F}}(\xPin,\kperp)
=
 F_{\mathrm{coll}}(\xPin,\kperp\big)
+F_{\mathrm{softcoll}}(\xPin,\kperp\big)
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
where
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
&F_{\mathrm{coll}}(\xPin,\kperp)=
    \frac{4\cNLO\Nc}{\vep}\bigg(\frac{\sTot\xPin(1-\xMin)}{\mu^2}\bigg)^{\vep/2}
    \int_{\xPin}^1\frac{dz}{(1-z)^{1-\vep/2}}
    \bigg[
    \frac{1}{z^{1+\vep/2}}
          \,F\bigg(\frac{\xPin}{z},\kperp\bigg)
         -F\big(\xPin,\kperp\big)
    \bigg]
\notag\\
&F_{\mathrm{softcoll}}(\xPin,\kperp)=
    \frac{8\cNLO\Nc}{\vep^2}\bigg(\frac{\sTot\xPin(1-\xPin)(1-\xMin)}{\mu^2}\bigg)^{\vep/2}
    F\big(\xPin,\kperp\big)
~.
\label{Eq:076}
\end{align}
%
The $z$-integral itself in \Equation{Eq:076} is finite for $\vep\to0$, but we also need $\Ord(\vep)$ because of the $1/\vep$ in front of the integral:
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
&F_{\mathrm{coll}}(\xPin,\kperp)=
    \frac{4\cNLO\Nc}{\vep}\bigg(\frac{\sTot\xPin(1-\xMin)}{\mu^2}\bigg)^{\vep/2}
\notag\\&\hspace{4ex}\times
    \Bigg\{
      \int_{\xPin}^1\frac{dz}{[1-z]_+}\,\frac{1}{z}
                    \,F\bigg(\frac{\xPin}{z},\kperp\bigg)
       +
      \frac{\vep}{2}\int_{\xPin}^1dz\,\frac{\ln(1-z)}{1-z}
               \bigg[
               \frac{1}{z}
                     \,F\bigg(\frac{\xPin}{z},\kperp\bigg)
                    -F\big(\xPin,\kperp\big)
               \bigg]
\notag\\&\hspace{40ex}
          -\frac{\vep}{2}
          \int_{\xPin}^1\frac{dz}{1-z}
             \frac{\ln z}{z}
                   \,F\bigg(\frac{\xPin}{z},\kperp\bigg)
    +\Ord\big(\vep^2\big)
    \Bigg\}
\label{Eq:077}
\end{align}
%
There is a $\ln\xPin$ hidden in the first integral of \Equation{Eq:077}.
%
We can write
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{multline}
\int_{\xPin}^1dz\,\frac{1}{[1-z]_+}\,\frac{1}{z}F\bigg(\frac{\xPin}{z},\kperp\bigg)
%=
%\int_{\xPin}^1dz\,\frac{1}{1-z}\bigg[\frac{1}{z}F\bigg(\frac{\xPin}{z},\kperp\bigg)-F(\xPin,\kperp)\bigg]
%\\
%=
%\int_{\xPin}^1\frac{dz}{z(1-z)}\bigg[F\bigg(\frac{\xPin}{z},\kperp\bigg)-F(\xPin,\kperp)\bigg]
%+
%\int_{\xPin}^1dz\,\frac{1}{1-z}\bigg[\frac{1}{z}-1\bigg]\,F(\xPin,\kperp)
\\
=
\int_{\xPin}^1\frac{dz}{z(1-z)}\bigg[F\bigg(\frac{\xPin}{z},\kperp\bigg)-F(\xPin,\kperp)\bigg]
+
\ln\bigg(\frac{1}{\xPin}\bigg)F(\xPin,\kperp)
%\ln\frac{1}{\xPin}\,\,F(\xPin,\kperp)
~.
\end{multline}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
The integral on the right-hand side does not generate $\ln\xPin$ anymore, as can easily be seen with the variable substitution $z=1/(1+y/\xPin)$:
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\int_{\xPin}^1\frac{dz}{z(1-z)}\bigg[F\bigg(\frac{\xPin}{z},\kperp\bigg)-F(\xPin,\kperp)\bigg]
=
\int_0^{1-\xPin}\frac{dy}{y}\bigg[F(\xPin+y,\kperp) - F(\xPin,\kperp)\bigg]
~.
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
The second integral in \Equation{Eq:077} does not generate $\ln\xPin$.
%
Instead, we get
%
\begin{multline}
\int_{\xPin}^1dz\,\frac{\ln(1-z)}{1-z}
               \bigg[
               \frac{1}{z}
                     \,F\bigg(\frac{\xPin}{z},\kperp\bigg)
                    -F\big(\xPin,\kperp\big)
               \bigg]
\\
=
\int_{\xPin}^1dz\,\frac{\ln(1-z)}{z(1-z)}
               \bigg[
                     \,F\bigg(\frac{\xPin}{z},\kperp\bigg)
                    -F\big(\xPin,\kperp\big)
               \bigg]
+
\bigg(\mathrm{Li}_2(\xPin)-\frac{\pi^2}{6}\bigg)\,F(\xPin,\kperp)
~.
\end{multline}
%
The third integral in \Equation{Eq:077}, finally, also does not generate $\ln\xPin$, because we may assume that $F(x,\kperp)$ vanishes if its first argument $x$ is not small, restricting the support for the integral to values of $z$ that are not far from $1$. 




